Categorification of the colored $\mathfrak{sl}_3$-invariant

We give explicit resolutions of all finite dimensional, simple $U_q(\mathfrak{sl_3})$-modules. We use these resolutions to categorify the colored $\mathfrak{sl}_3$-invariant of framed links via a complex of complexes of graded $\mathbb{Z}$-modules.

==> c3_exampleYtrefoil.tex <==
\begin{scope}[scale=0.7]
\draw[draw=  gray, line width = 2mm] (-2.75,2.5) --  (14.5,2.5); 
\draw[draw=  gray, line width = 2mm] (-2.75,-2.3) --  (14.5,-2.3); 
\draw[draw=  gray, very thick] (-2.75,-2.3) -- +(0,4.8);
\draw[draw=  gray, very thick] (2.75,-2.3) -- +(0,4.8);
\draw[draw=  gray, very thick] (8.5,-2.3) -- +(0,4.8);
\draw[draw=  gray, very thick] (14,-2.3) -- +(0,4.8);
\draw[draw= white, dotted, line width =1.2mm] (-2.75,2.5) --  (14.5,2.5); 
\draw[draw= white, dotted, line width = 1.2mm] (-2.75,-2.3) --  (14.5,-2.3); 

\begin{scope}[yshift= -6cm]
\draw[draw=  gray, line width = 2mm] (-3.25,2.5) --  (14.5,2.5); 
\draw[draw=  gray, line width = 2mm] (-3.25,-2.3) --  (14.5,-2.3); 
\draw[draw=  gray, very thick] (-2.75,-2.3) -- +(0,4.8);
\draw[draw=  gray, very thick] (2.75,-2.3) -- +(0,4.8);
\draw[draw=  gray, very thick] (8.5,-2.3) -- +(0,4.8);
\draw[draw=  gray, very thick] (14,-2.3) -- +(0,4.8);
\draw[draw= white, dotted, line width =1.2mm] (-3.25,2.5) --  (14.5,2.5); 
\draw[draw= white, dotted, line width = 1.2mm] (-3.25,-2.3) --  (14.5,-2.3); 
\end{scope}

\begin{scope}[yshift= -12cm]
\draw[draw=  gray, line width = 2mm] (-3.25,2.5) --  (14,2.5); 
\draw[draw=  gray, line width = 2mm] (-3.25,-2.3) --  (14,-2.3); 
\draw[draw=  gray, very thick] (-2.75,-2.3) -- +(0,4.8);
\draw[draw=  gray, very thick] (2.75,-2.3) -- +(0,4.8);
\draw[draw=  gray, very thick] (8.5,-2.3) -- +(0,4.8);
\draw[draw=  gray, very thick] (14,-2.3) -- +(0,4.8);
\draw[draw= white, dotted, line width =1.2mm] (-3.25,2.5) --  (14,2.5); 
\draw[draw= white, dotted, line width = 1.2mm] (-3.25,-2.3) --  (14,-2.3); 
\end{scope}

\begin{scope}[xshift=0cm]
\begin{knot}[ consider self intersections,
 flip crossing=3,
 flip crossing=5,
 flip crossing=4,
 flip crossing=7,
 flip crossing=9,
 flip crossing=11,
 clip width=3,
]
\strand
(90:2) to[out=180,in=-120,looseness=2]
(-30:2) to[out=60,in=120,looseness=2]
(210:2) to[out=-60,in=0,looseness=2] (90:2);
 \strand
 (90:1.8) to[out=180,in=-120,looseness=1.8]
 (-30:1.8) to[out=60,in=120,looseness=1.8]
 (210:1.8) to[out=-60,in=0,looseness=1.8] (90:1.8);
\end{knot}  
\end{scope}

\begin{scope}[xshift=5.5cm]
\begin{knot}[ consider self intersections,
 flip crossing=3,
 flip crossing=5,
 flip crossing=4,
 flip crossing=7,
 flip crossing=9,
 flip crossing=12,
clip width=3,
]
\strand
(90:2) to[out=180,in=-120,looseness=2]
(-30:2) to[out=60,in=120,looseness=2]
(210:2) to[out=-60,in=0,looseness=2] (90:2);
 \strand
 (100:1.8) to[out=190,in=-120,in looseness=1.7, out looseness = 1.2]
 (-30:1.8) to[out=60,in=120,looseness=1.8]
 (210:1.8) to[out=-60,in=-10,out looseness=1.7, in looseness = 1.2] (80:1.8);
\end{knot}  
\draw (100:1.8) to [out= 10, in= - 185, looseness = 1] (95: 2);
\draw (80:1.8) to [out= 170, in= -5, looseness = 1] (85: 2);
\end{scope}

\begin{scope}[xshift=11cm]
\begin{knot}[ consider self intersections,
 flip crossing=1,
 flip crossing=5,
 flip crossing=4,
 flip crossing=8,
clip width=3,
]
\strand
(90:2) to[out=180,in=-120,looseness=2]
(-30:2) to[out=60,in=120,looseness=2]
(210:2) to[out=-60,in=0,looseness=2] (90:2);
 \strand
 (250:0.65) to[out=-60,in=-120,in looseness=1.7, out looseness = 0.5]
 (-30:1.8) to[out=60,in=120,looseness=1.8]
 (210:1.8) to[out=-60,in=-10,out looseness=1.7, in looseness = 1.2] (80:1.8);
\end{knot}  
\draw (250:0.65) to [out= 120, in= -45, looseness = 1] (220:0.76);
\draw (80:1.8) to [out= 170, in= -5, looseness = 1] (85: 2);
\end{scope}

\begin{scope}[xshift=0cm, yshift= -6cm]
\begin{knot}[
 flip crossing=7,
 flip crossing=2,
 flip crossing=4,
 clip width=3, 
]
\strand (90:2) to[out=180,in=-120,looseness=2] (-30:2); 
\strand (-30:2) to[out=60,in=120,looseness=2](210:2);
\strand (210:2) to[out=-60,in=0,looseness=2] (90:2);
 \strand  (-20:1.8) to[out=60,in=120,out looseness=1.2, in looseness = 1.8] (210:1.8);
\strand
 (210:1.8) to[out=-60,in=0, in looseness=1.1, out looseness= 1.8] (80:1.8);
\end{knot} 
\draw (-20:1.8) to [out= -110, in= - 305, looseness = 1] (-25: 2);
\draw (80:1.8) to [out= 170, in= -5, looseness = 1] (85: 2);
\end{scope}

\begin{scope}[xshift=5.5cm, yshift= -6cm]
\begin{knot}[
 flip crossing=2,
 flip crossing=3,
 flip crossing=6,
 clip width=3,
]
\strand (90:2) to[out=180,in=-120,looseness=2] (-30:2); 
\strand (-30:2) to[out=60,in=120,looseness=2](210:2);
\strand (210:2) to[out=-60,in=0,looseness=2] (90:2);
 \strand
 (130:0.65) to[out=-180,in=120,in looseness=1.7, out looseness = 0.5]  (210:1.8);
\strand (210:1.8) to[out=-60,in=0, in looseness=1.1, out looseness= 1.8] (80:1.8);
\end{knot}  
\draw (130:0.65) to [out= 0, in= -185, looseness = 1] (100:0.762);
\draw (80:1.8) to [out= 170, in= -5, looseness = 1] (85: 2);
\end{scope}

\begin{scope}[xshift=11cm, yshift= -6cm]
\begin{knot}[ %consider self intersections,
% flip crossing=1,
 flip crossing=2,
 flip crossing=3,
% flip crossing=5,
% flip crossing=4,
% flip crossing=7,
% flip crossing=9,
% flip crossing=11,
 clip width=3,
]
\strand (90:2) to[out=180,in=-120,looseness=2] (-30:2); 
\strand (-30:2) to[out=60,in=120,looseness=2](210:2);
\strand (210:2) to[out=-60,in=0,looseness=2] (90:2);
 \strand
% (90:1.8) to[out=180,in=-120,looseness=1.8]
% (-30:1.8) to[out=60,in=120,looseness=1.8]
 (210:1.8) to[out=-60,in=0, in looseness=1.1, out looseness= 1.8] (80:1.8);
\end{knot}  
\draw (-150:1.8) to [out= 120, in= - 65, looseness = 1] (-160: 2);
\draw (80:1.8) to [out= 170, in= -5, looseness = 1] (85: 2);
\end{scope}



\begin{scope}[xshift=0cm, yshift= -12cm]
\begin{knot}[ %consider self intersections,
 flip crossing=2,
 flip crossing=5,
 clip width=3,
]
\strand (90:2) to[out=180,in=-120,looseness=2] (-30:2); 
\strand (-30:2) to[out=60,in=120,looseness=2](210:2);
\strand (210:2) to[out=-60,in=0,looseness=2] (90:2);
 \strand
% (90:1.8) to[out=180,in=-120,looseness=1.8]
% (100:1.8) to[out=190,in=-120,in looseness=1.7, out looseness = 1.2]
% (-30:1.8) to[out=60,in=120,looseness=1.8]
 (10:0.65) to[out=60,in=0,in looseness=0.7, out looseness = 1.1] (80:1.8);
\end{knot}  
\draw (10:0.65) to [out= -120, in= 110, looseness = 1] (-20:0.762);
\draw (80:1.8) to [out= 170, in= -5, looseness = 1] (85: 2);
\end{scope}

\begin{scope}[xshift=5.5cm, yshift= -12cm]
\begin{knot}[ consider self intersections,
% flip crossing=1,
 flip crossing=2,
% flip crossing=3,
 clip width=3,
]
\strand
(90:2) to[out=180,in=-120,looseness=2]
(-30:2) to[out=60,in=120,looseness=2]
(210:2) to[out=-60,in=0,looseness=2] (90:2);
 \strand
 (60:1.6) to[out=100,in=0,in looseness=0.7, out looseness = 1.1] (80:1.8);
\end{knot}  
\draw (60:1.6) to [out= 280, in= 800, looseness = 1] (50:1.6);
\draw (80:1.8) to [out= 170, in= -5, looseness = 1] (85: 2);
\end{scope}

\begin{scope}[xshift=11cm, yshift= -12cm]
\begin{knot}[ consider self intersections,
% flip crossing=1,
 flip crossing=2,
 % flip crossing=3,
 % flip crossing=5,
 % flip crossing=4,
 % flip crossing=7,
 % flip crossing=9,
 % flip crossing=11,
 clip width=3,
]
\strand
(90:2) to[out=180,in=-120,looseness=2]
(-30:2) to[out=60,in=120,looseness=2]
(210:2) to[out=-60,in=0,looseness=2] (90:2);
\end{knot}
\end{scope}
\end{scope}



==> c3_examplenutrefoil.tex <==
\begin{scope}[scale=0.7]
\draw[draw=  gray, line width = 2mm] (-2.75,2.5) --  (14.5,2.5); 
\draw[draw=  gray, line width = 2mm] (-2.75,-2.3) --  (14.5,-2.3); 
\draw[draw=  gray, very thick] (-2.75,-2.3) -- +(0,4.8);
\draw[draw=  gray, very thick] (2.75,-2.3) -- +(0,4.8);
\draw[draw=  gray, very thick] (8.5,-2.3) -- +(0,4.8);
\draw[draw=  gray, very thick] (14,-2.3) -- +(0,4.8);
\draw[draw= white, dotted, line width =1.2mm] (-2.75,2.5) --  (14.5,2.5); 
\draw[draw= white, dotted, line width = 1.2mm] (-2.75,-2.3) --  (14.5,-2.3); 

\begin{scope}[yshift= -6cm]
\draw[draw=  gray, line width = 2mm] (-3.25,2.5) --  (14.5,2.5); 
\draw[draw=  gray, line width = 2mm] (-3.25,-2.3) --  (14.5,-2.3); 
\draw[draw=  gray, very thick] (-2.75,-2.3) -- +(0,4.8);
\draw[draw=  gray, very thick] (2.75,-2.3) -- +(0,4.8);
\draw[draw=  gray, very thick] (8.5,-2.3) -- +(0,4.8);
\draw[draw=  gray, very thick] (14,-2.3) -- +(0,4.8);
\draw[draw= white, dotted, line width =1.2mm] (-3.25,2.5) --  (14.5,2.5); 
\draw[draw= white, dotted, line width = 1.2mm] (-3.25,-2.3) --  (14.5,-2.3); 
\end{scope}

\begin{scope}[yshift= -12cm, xshift = -2.75cm]
\draw[draw=  gray, line width = 2mm] (2.25,2.5) --  (14,2.5); 
\draw[draw=  gray, line width = 2mm] (2.25,-2.3) --  (14,-2.3); 
\draw[draw=  gray, very thick] (2.75,-2.3) -- +(0,4.8);
\draw[draw=  gray, very thick] (8.5,-2.3) -- +(0,4.8);
\draw[draw=  gray, very thick] (14,-2.3) -- +(0,4.8);
\draw[draw= white, dotted, line width =1.2mm] (2.25,2.5) --  (14,2.5); 
\draw[draw= white, dotted, line width = 1.2mm] (2.25,-2.3) --  (14,-2.3); 
\end{scope}

\begin{scope}[xshift=0cm]
\begin{knot}[ consider self intersections,
 flip crossing=3,
 flip crossing=5,
 flip crossing=4,
 flip crossing=7,
 flip crossing=9,
 flip crossing=11,
 clip width=3,
]
\strand
(90:2) to[out=180,in=-120,looseness=2]
(-30:2) to[out=60,in=120,looseness=2]
(210:2) to[out=-60,in=0,looseness=2] (90:2);
 \strand
 (90:1.8) to[out=180,in=-120,looseness=1.8]
 (-30:1.8) to[out=60,in=120,looseness=1.8]
 (210:1.8) to[out=-60,in=0,looseness=1.8] (90:1.8);
\end{knot}  
\end{scope}

\begin{scope}[xshift=5.5cm]
\begin{knot}[ 
 flip crossing=7,
 flip crossing=8,
clip width=3,
]
\strand (100:2) to[out=190,in=-120,looseness=1.7] (-30:2); 
\strand (100:1.8) to[out=190,in=-120,looseness=1.5] (-30:1.8); 
\strand (-30:2) to[out=60,in=120,looseness=2] (210:2);
\strand (-30:1.8) to[out=60,in=120,looseness=1.8] (210:1.8); 
\strand (210:2) to[out=-60,in=-10,looseness=1.7] (80:2);
\strand (210:1.8) to[out=-60,in=-10,looseness=1.5] (80:1.8);
\end{knot}  
\draw (100:2) .. controls +(10:0.2) and +(10:0.2) .. (100:1.8);
\draw (80:2) .. controls +(170:0.2) and +(170:0.2) .. (80:1.8);
\end{scope}

\begin{scope}[xshift=11cm]
\begin{knot}[
 flip crossing=1,
 flip crossing=2,
 flip crossing=4,
 flip crossing=3,
clip width=3,
]
\strand (210:0.85) to[out=-60,in=-120, in looseness=2, out looseness = 0.5] (-30:2) ;
\strand  (210:0.65) to[out=-60,in=-120,in looseness=1.8, out looseness = 0.5]  (-30:1.8); 
\strand (-30:2) to[out=60,in=120,looseness=2] (210:2); 
\strand  (-30:1.8) to[out=60,in=120,looseness=1.8] (210:1.8); 
\strand (210:2) to[out=-60,in=0,out looseness=2, in looseness= 1.4] (80:2);
\strand  (210:1.8) to[out=-60,in=-10,out looseness=1.8, in looseness = 1.2] (80:1.8);
\end{knot}  
\draw (210:0.85) .. controls +(120:0.2) and +(120:0.2) .. (210:0.65);
\draw (80:2) .. controls +(170:0.2) and +(170:0.2) .. (80:1.8);
\end{scope}

\begin{scope}[xshift=0cm, yshift= -6cm]
\begin{knot}[ clip width=3, 
]
\strand  (-20:2) to[out=60,in=120,out looseness=1.4, in looseness = 2] (210:2);
\strand  (-20:1.8) to[out=60,in=120,out looseness=1.2, in looseness = 1.8] (210:1.8);
\strand  (210:2) to[out=-60,in=0, in looseness=1.3, out looseness= 2] (80:2);
\strand  (210:1.8) to[out=-60,in=0, in looseness=1.1, out looseness= 1.8] (80:1.8);
\end{knot} 
\draw (-20:2) .. controls +(-120:0.2) and +(-120:0.2) .. (-20:1.8);
\draw (80:2) .. controls +(170:0.2) and +(170:0.2) .. (80:1.8);
\end{scope}

\begin{scope}[xshift=5.5cm, yshift= -6cm]
\begin{knot}[
 flip crossing=2,
 flip crossing=3,
 flip crossing=6,
 clip width=3,
]
 \strand  (130:0.85) to[out=-180,in=120,in looseness=2, out looseness = 0.7]  (210:2);
\strand (210:2) to[out=-60,in=0, in looseness=1.3, out looseness= 2] (80:2);
 \strand  (130:0.65) to[out=-180,in=120,in looseness=1.7, out looseness = 0.5]  (210:1.8);
\strand (210:1.8) to[out=-60,in=0, in looseness=1.1, out looseness= 1.8] (80:1.8);
\end{knot}  
\draw (130:0.85) .. controls +(0:0.3) and +(0:0.2) .. (130:0.65);
\draw (80:2) .. controls +(170:0.2) and +(170:0.2) .. (80:1.8);
\end{scope}

\begin{scope}[xshift=11cm, yshift= -6cm]
\begin{knot}[
]
\strand (210:2) to[out=-60,in=0, in looseness=1.3, out looseness= 2] (80:2);
\strand (210:1.8) to[out=-60,in=0, in looseness=1.1, out looseness= 1.8] (80:1.8);
\end{knot}  
\draw (210:2) .. controls +(120:0.2) and +(120:0.2) .. (210:1.8);
\draw (80:2) .. controls +(170:0.2) and +(170:0.2) .. (80:1.8);
\end{scope}

\begin{scope}[xshift=2.75cm, yshift= -12cm]
\draw (80:2) .. controls +(-10:0.2) and +(-10:0.2) .. (80:1.8);
\draw (80:2) .. controls +(170:0.2) and +(170:0.2) .. (80:1.8);
\end{scope}


\end{scope}


